Energy-Aware FPGA Implementation of Spiking Neural Network with LIF Neurons

Tiny Machine Learning (TinyML) has become a growing field in on-device processing for Internet of Things (IoT) applications, capitalizing on AI algorithms that are optimized for their low complexity and energy efficiency. These algorithms are designed to minimize power and memory footprints, making them ideal for the constraints of IoT devices. Within this domain, Spiking Neural Networks (SNNs) stand out as a cutting-edge solution for TinyML, owning to their event-driven processing paradigm which offers an efficient method of handling dataflow. This paper presents a novel SNN architecture based on the 1st Order Leaky Integrate-and-Fire (LIF) neuron model to efficiently deploy vision-based ML algorithms on TinyML systems. A hardware-friendly LIF design is also proposed, and implemented on a Xilinx Artix-7 FPGA. To evaluate the proposed model, a collision avoidance dataset is considered as a case study. The proposed SNN model is compared to the state-of-the-art works and Binarized Convolutional Neural Network (BCNN) as a baseline. The results show the proposed approach is 86% more energy efficient than the baseline.

==> Hardware_implementation.tex <==
\section{Hardware Implementation}
\label{sec:Hardware_Implementation}

The implementation of the Spiking Neural Network (SNN) architecture on a Field-Programmable Gate Array (FPGA) involves a novel approach that leverages the unique characteristics of FPGAs for efficient neural computation. This section outlines the key aspects of this implementation, focusing on the representation of neural network parameters and the design of the hardware architecture.

\begin{itemize}
    \item Signed Q1.7 Format: The weights, biases, and neuron states in the SNN are represented using an 8-bit signed fixed-point format, known as Q1.7. This format allows for a range from -1 to approximately +0.992.
\item Range Considerations: Due to the constraints of the Q1.7 format, all neural network calculations are confined within the -1 to +1 range. This limitation ensures that the data representation is consistent and avoids overflow or underflow errors in computations.
\end{itemize}

\begin{figure}[!htbp]
    \centering
    \scalebox{1}{
    \includesvg[width=0.47\textwidth]{Figures/NHU_Cascaded_Adder_SNN.svg}}
    \caption{Proposed hardware architecture for SNN.}
    \label{fig:hardware_architecture}
\end{figure}

\subsection{Hardware Architecture}
\subsubsection{Cascaded Adder}
\begin{itemize}
\item Binary Pixel Values: Given that the input pixel values are binary (0 or 1), the standard matrix multiplication operation common in neural networks is simplified.
Adder Tree: A cascaded adder, or adder tree, replaces the need for multipliers, which are traditionally more resource-intensive on silicon. This substitution significantly reduces the hardware complexity and power consumption.
\item Bias Addition: The addition of bias values to the neurons is performed after the cascaded adder computation, maintaining the integrity of the neural network's functionality.
\end{itemize}

\subsection{Neuron Hardware Unit (NHU)}


The Neuron Hardware Unit (NHU) is an integral part of the FPGA-based Spiking Neural Network architecture, designed to emulate the dynamic behavior of biological neurons in a digital framework. Its primary functionality revolves around processing input signals, accumulating them over time, and generating an output spike under certain conditions, akin to a neuron firing in response to stimuli.

The NHU simulates the neuron's response to stimuli, where input signals are accumulated until a threshold is reached, leading to a spike. This process mirrors the all-or-nothing firing mechanism of biological neurons. The use of a threshold in determining the firing of the neuron is significant. It ensures that the NHU only generates a spike when the accumulated input is sufficiently strong, thereby mimicking the selective response of neurons in the brain. The reset of a spike is a crucial aspect of the NHU, as it models the refractory period in biological neurons. This mechanism prevents immediate re-firing, ensuring a realistic emulation of neuronal behavior.
